Iteration Complexity and Finite-Time Efficiency of Adaptive Sampling Trust-Region Methods for Stochastic Derivative-Free Optimization

Adaptive sampling with interpolation-based trust regions or ASTRO-DF is a successful algorithm for stochastic derivative-free optimization with an easy-to-understand-and-implement concept that guarantees almost sure convergence to a first-order critical point. To reduce its dependence on the problem dimension, we present local models with diagonal Hessians constructed on interpolation points based on a coordinate basis. We also leverage the interpolation points in a direct search manner whenever possible to boost ASTRO-DF's performance in a finite time. We prove that the algorithm has a canonical iteration complexity of $\mathcal{O}(\epsilon^{-2})$ almost surely, which is the first guarantee of its kind without placing assumptions on the quality of function estimates or model quality or independence between them. Numerical experimentation reveals the computational advantage of ASTRO-DF with coordinate direct search due to saving and better steps in the early iterations of the search.

==> mycommands.tex <==

%%% EDITING SHORTCUTS -----------------------------------------------------------------------------

%\newcommand{\sara}[1]{{\color{red}{\textbf{[SS: #1]}}\color{black}}}
%\newcommand{\stopped}{ \[=======================================================\]}
%\newcommand{\done}{We agree. Done, thank you.}
%\newcommand{\yunsoo}[1]{{\color{blue}{\textbf{[HA: #1]}}\color{black}}}
%\newcommand{\annot}[1]{{\text{\normalfont #1}}}

%%% TEACHING SHORTCUTS -----------------------------------------------------------------------------

\newcommand{\answerblank}[1]{\underline{\makebox[#1][l]{ }}}

%%% MATH SHORTCUTS -----------------------------------------------------------------------------

% BEGIN: THIS CODE DEFINES THE \widebar COMMAND, WITH ADJUSTMENTS 

\makeatletter
\let\save@mathaccent\mathaccent
\newcommand*\if@single[3]{%
  \setbox0\hbox{${\mathaccent"0362{#1}}^H$}%
  \setbox2\hbox{${\mathaccent"0362{\kern0pt#1}}^H$}%
  \ifdim\ht0=\ht2 #3\else #2\fi
  }
%The bar will be moved to the right by a half of \macc@kerna, which is computed by amsmath:
\newcommand*\rel@kern[1]{\kern#1\dimexpr\macc@kerna}
%If there's a superscript following the bar, then no negative kern may follow the bar;
%an additional {} makes sure that the superscript is high enough in this case:
\newcommand*\widebar[1]{\@ifnextchar^{{\wide@bar{#1}{0}}}{\wide@bar{#1}{1}}}
%Use a separate algorithm for single symbols:
\newcommand*\wide@bar[2]{\if@single{#1}{\wide@bar@{#1}{#2}{1}}{\wide@bar@{#1}{#2}{2}}}
\newcommand*\wide@bar@[3]{%
  \begingroup
  \def\mathaccent##1##2{%
%Enable nesting of accents:
    \let\mathaccent\save@mathaccent
%If there's more than a single symbol, use the first character instead (see below):
    \if#32 \let\macc@nucleus\first@char \fi
%Determine the italic correction:
    \setbox\z@\hbox{$\macc@style{\macc@nucleus}_{}$}%
    \setbox\tw@\hbox{$\macc@style{\macc@nucleus}{}_{}$}%
    \dimen@\wd\tw@
    \advance\dimen@-\wd\z@
%Now \dimen@ is the italic correction of the symbol.
    \divide\dimen@ 3
    \@tempdima\wd\tw@
    \advance\@tempdima-\scriptspace
%Now \@tempdima is the width of the symbol.
    \divide\@tempdima 10
    \advance\dimen@-\@tempdima
%Now \dimen@ = (italic correction / 3) - (Breite / 10)
    \ifdim\dimen@>\z@ \dimen@0pt\fi
%The bar will be shortened in the case \dimen@<0 !
    \rel@kern{0.6}\kern-\dimen@
    \if#31
      \overline{\rel@kern{-0.6}\kern\dimen@\macc@nucleus\rel@kern{0.4}\kern\dimen@}%
      \advance\dimen@0.4\dimexpr\macc@kerna
%Place the combined final kern (-\dimen@) if it is >0 or if a superscript follows:
      \let\final@kern#2%
      \ifdim\dimen@<\z@ \let\final@kern1\fi
      \if\final@kern1 \kern-\dimen@\fi
    \else
      \overline{\rel@kern{-0.6}\kern\dimen@#1}%
    \fi
  }%
  \macc@depth\@ne
  \let\math@bgroup\@empty \let\math@egroup\macc@set@skewchar
  \mathsurround\z@ \frozen@everymath{\mathgroup\macc@group\relax}%
  \macc@set@skewchar\relax
  \let\mathaccentV\macc@nested@a
%The following initialises \macc@kerna and calls \mathaccent:
  \if#31
    \macc@nested@a\relax111{#1}%
  \else
%If the argument consists of more than one symbol, and if the first token is
%a letter, use that letter for the computations:
    \def\gobble@till@marker##1\endmarker{}%
    \futurelet\first@char\gobble@till@marker#1\endmarker
    \ifcat\noexpand\first@char A\else
      \def\first@char{}%
    \fi
    \macc@nested@a\relax111{\first@char}%
  \fi
  \endgroup
}
\makeatother
% END: THIS CODE DEFINES THE \widebar COMMAND, WITH ADJUSTMENTS 


%argmin and argmax
\DeclareMathOperator*{\argmin}{\arg\!\min}
\DeclareMathOperator*{\argmax}{\arg\!\max}

%real numbers
\newcommand{\real}{{\rm{I\hspace{-.75mm}R}}}
\newcommand{\ereal}{\widebar{\real}}

%operations
\newcommand{\domeq}{\preceq} %dominates, for multi-obj. work
\newcommand{\dom}{\prec}
\newcommand{\ndom}{\nprec}
\newcommand{\indic}[1]{\mathbb I\{#1\}}


%sums and products
\newcommand{\sumin}{\sum_{i=1}^n}
\newcommand{\sumir}{\sum_{i=1}^r}
\newcommand{\smsum}{\mathop{\textstyle\sum}}
\newcommand{\smsumin}{\mathop{\textstyle\sum}_{i=1}^n}
\newcommand{\smsumir}{\mathop{\textstyle\sum}_{i=1}^r}
\newcommand{\smprod}{\mathop{\textstyle\prod}}
\newcommand{\prodin}{\prod_{i=1}^n}

%fractions
\newcommand{\oon}{\frac{1}{n}} 
\newcommand{\oom}{\frac{1}{m}}
\newcommand{\oot}{\frac{1}{t}}
\newcommand{\oo}[1]{\frac{1}{#1}}
\newcommand{\ootwo}{\frac{1}{2}}
%\newcommand{\onehalf}[1]{\frac{#1}{2}}

\newcommand{\sqrtn}{\sqrt{n}}

%limits
\newcommand{\limn}{\lim_{n\rightarrow\infty}}
\newcommand{\limt}{\lim_{t\rightarrow\infty}}
\newcommand{\limnstack}{\displaystyle\lim_{n\rightarrow\infty}\textstyle}

%Statistical quantities and expressions
\renewcommand*{~}{\relax\ifmmode\sim\else\nobreakspace{}\fi}%GET TILDE FOR "IS DISTRIBUTED AS"
\newcommand{\Expect}{\mbox{{\normalfont E}}}
\newcommand{\Ex}{{\rm{I\hspace{-.75mm}E}}}
\newcommand{\se}{\mbox{s.e.}}
\newcommand{\sehat}{\widehat{\mbox{s.e.}}}
\newcommand{\Var}{\mbox{Var}}
\newcommand{\Varhat}{\widehat{\mbox{Var}}}
\newcommand{\Cov}{\mbox{Cov}}
\newcommand{\Covhat}{\widehat{\mbox{Cov}}}
\newcommand{\Corr}{\mbox{Corr}}
\newcommand{\mse}{\mbox{mse}}
\newcommand{\PFS}{P\{\mbox{FS}\}}
\newcommand{\PFSi}{P\{\mbox{FS}_i\}}
\newcommand{\PCS}{P\{\mbox{CS}\}}

\newcommand{\evalat}{\biggl.\biggr|}

%parentheses
\newcommand{\lpr}{\left(}     \newcommand{\rpr}{\right)}
\newcommand{\lcbr}{\left\{}  \newcommand{\rcbr}{\right\}}
\newcommand{\lbr}{\left[}     \newcommand{\rbr}{\right]}
\newcommand{\ld}{\left.}      \newcommand{\rd}{\right.}

\newcommand{\abs}[1]{\lvert #1 \rvert}
\newcommand{\norm}[1]{\lVert #1 \rVert}

%mbox shortcuts
\newcommand{\myand}{\quad\mbox{and}\quad}
\newcommand{\myor}{\quad\mbox{or}\quad}
\newcommand{\myif}{\mbox{if }}
\newcommand{\myfor}{\mbox{for }}
\newcommand{\mywp}{\mbox{w.p. }}


%%% FORMATTING SHORTCUTS -----------------------------------------------------------------------------

\newcommand{\thme}[2]{{\begin{theorem}[#1]#2\end{theorem}}}
\newcommand{\prope}[2]{{\begin{proposition}[#1]#2\end{proposition}}}
\newcommand{\leme}[2]{{\begin{lemma}[#1]#2\end{lemma}}}
\newcommand{\core}[2]{{\begin{corollary}[#1]#2\end{corollary}}}
\newcommand{\resulte}[2]{{\begin{result}[#1]#2\end{result}}}
\newcommand{\assume}[2]{{\begin{assumption}[#1]#2\end{assumption}}}
\newcommand{\remarke}[2]{{\begin{remark}[#1]#2\end{remark}}}
\newcommand{\defne}[2]{\begin{definition}[#1]#2\end{definition}}
\newcommand{\exe}[2]{{\begin{example}[#1]#2\end{example}}}
\newcommand{\myproof}[2]{{\begin{proof}[#1]#2\end{proof}}}

\newenvironment{itemizec}
{ \begin{itemize}[nosep]    }
{ \end{itemize}                  } 

%%% LETTERS -----------------------------------------------------------------------------

%STATISTICAL LETTERS

%BARS -------------------------
%bars: roman
\newcommand{\Bbar}{\bar{B}}
\newcommand{\Ebar}{\bar{E}}
\newcommand{\Fbar}{\bar{F}}
\newcommand{\Gbar}{\bar{G}}
\newcommand{\Hbar}{\bar{H}}
\newcommand{\Lbar}{\bar{L}}
\newcommand{\Xbar}{\bar{X}}
\newcommand{\Ybar}{\bar{Y}}
\newcommand{\fbar}{\bar{f}}
\newcommand{\gbar}{\bar{g}}
% \newcommand{\hbar}{\bar{h}}
%bars: greek
\newcommand{\Gammabar}{\bar{\Gamma}}
\newcommand{\Phibar}{\bar{\Phi}}

%HATS -------------------------
%hats: roman
\newcommand{\bhat}{\hat{b}}
\newcommand{\chat}{\hat{c}}
\newcommand{\fhat}{\hat{f}}
\newcommand{\ellhat}{\hat{\ell}}
\newcommand{\mhat}{\hat{m}}
\newcommand{\phat}{\hat{p}}
\newcommand{\shat}{\hat{s}}
\newcommand{\what}{\hat{w}}
\newcommand{\yhat}{\hat{y}}
\newcommand{\Bhat}{\hat{B}}
\newcommand{\Dhat}{\hat{D}}
\newcommand{\Fhat}{\hat{F}}
\newcommand{\Ghat}{\hat{G}}
\newcommand{\Hhat}{\hat{H}}
\newcommand{\Ihat}{\hat{I}}
\newcommand{\Jhat}{\hat{J}}
\newcommand{\Lhat}{\hat{L}}
\newcommand{\Mhat}{\hat{M}}
\newcommand{\Nhat}{\hat{N}}
\newcommand{\Phat}{\hat{P}}
\newcommand{\Qhat}{\hat{Q}}
\newcommand{\Rhat}{\hat{R}}
\newcommand{\Shat}{\hat{S}}
\newcommand{\Vhat}{\hat{V}}
\newcommand{\Xhat}{\hat{X}}
\newcommand{\Yhat}{\hat{Y}}
%hats: greek
\newcommand{\alphahat}{\hat{\alpha}}
\newcommand{\betahat}{\hat{\beta}}
\newcommand{\varepsilonhat}{\hat{\varepsilon}}
\newcommand{\lambdahat}{\hat{\lambda}}
\newcommand{\muhat}{\hat{\mu}}
\newcommand{\rhohat}{\hat{\rho}}
\newcommand{\sigmahat}{\hat{\sigma}}
\newcommand{\thetahat}{\hat{\theta}}
\newcommand{\Gammahat}{\widehat{\Gamma}}
\newcommand{\Sigmahat}{\widehat{\Sigma}}

%TILDE -------------------------
\newcommand{\gtilde}{\tilde{g}}
\newcommand{\ztilde}{\tilde{z}}
\newcommand{\Xtilde}{\widetilde{X}}
\newcommand{\Gtilde}{\widetilde{G}}
\newcommand{\Ntilde}{\widetilde{N}}
\newcommand{\Qtilde}{\widetilde{Q}}
\newcommand{\Rtilde}{\widetilde{R}}
\newcommand{\Ftilde}{\widetilde{F}}
%tilde: greek
\newcommand{\alphatilde}{\tilde{\alpha}}
\newcommand{\Deltatilde}{\widetilde{\Delta}}


%CHECK -------------------------
\newcommand{\Ncheck}{\check{N}}
\newcommand{\BFXcheck}{\check{\BFX}}


%BOLDFACE -- for compatibility with INFORMS formats
%roman LOWER
\newcommand{\BFa}{\bm{a}}
\newcommand{\BFb}{\bm{b}}
\newcommand{\BFc}{\bm{c}}
\newcommand{\BFd}{\bm{d}}
\newcommand{\BFe}{\bm{e}}
\newcommand{\BFf}{\bm{f}}
\newcommand{\BFg}{\bm{g}}
\newcommand{\BFh}{\bm{h}}
\newcommand{\BFp}{\bm{p}}
\newcommand{\BFs}{\bm{s}}
\newcommand{\BFt}{\bm{t}}
\newcommand{\BFu}{\bm{u}}
\newcommand{\BFw}{\bm{w}}
\newcommand{\BFx}{\bm{x}}
\newcommand{\BFy}{\bm{y}}
\newcommand{\BFz}{\bm{z}}
%roman UPPER
\newcommand{\BFE}{\bm{E}}
\newcommand{\BFF}{\bm{F}}
\newcommand{\BFG}{\bm{G}}
\newcommand{\BFH}{\bm{H}}
\newcommand{\BFP}{\bm{P}}
\newcommand{\BFW}{\bm{W}}
\newcommand{\BFU}{\bm{U}}
\newcommand{\BFX}{\bm{X}}
\newcommand{\BFS}{\bm{S}}
\newcommand{\BFY}{\bm{Y}}
\newcommand{\BFZ}{\bm{Z}}
%greek
\newcommand{\BFalpha}{\bm{\alpha}}
\newcommand{\BFbeta}{\bm{\beta}}
\newcommand{\BFdelta}{\bm{\delta}}
\newcommand{\BFDelta}{\bm{\Delta}}
\newcommand{\BFepsilon}{\bm{\epsilon}}
\newcommand{\BFvarepsilon}{{\bm{\varepsilon}}}
\newcommand{\BFtheta}{\bm{\theta}}
\newcommand{\BFgamma}{\bm{\gamma}}
\newcommand{\BFlambda}{\bm{\lambda}}
\newcommand{\BFLambda}{\bm{\Lambda}}
\newcommand{\BFnu}{\bm{\nu}}
\newcommand{\BFmu}{\bm{\mu}}
\newcommand{\BFomega}{\bm{\omega}}
\newcommand{\BFOmega}{\bm{\Omega}}
\newcommand{\BFrho}{\bm{\rho}}
%symbols
\newcommand{\BFzero}{\bm{0}}
\newcommand{\BFinfty}{\bm{\infty}}


%TWO OR MORE MODIFICATIONS

%bold and bar: roman
\newcommand{\BFybar}{\bar{\BFy}}
\newcommand{\BFEbar}{\bar{\BFE}}
\newcommand{\BFFbar}{\bar{\BFF}}
\newcommand{\BFGbar}{\bar{\BFG}}
\newcommand{\BFXbar}{\bar{\BFX}}
\newcommand{\BFYbar}{\bar{\BFY}}

%bold and hat: roman
\newcommand{\BFGhat}{\hat{\BFG}}
\newcommand{\BFHhat}{\hat{\BFH}}
\newcommand{\BFXhat}{\hat{\BFX}}
\newcommand{\BFYhat}{\hat{\BFY}}
%bold and hat: greek
\newcommand{\BFalphahat}{\hat{\BFalpha}}
\newcommand{\BFvarepsilonhat}{\hat{\BFvarepsilon}}
\newcommand{\BFthetahat}{\hat{\BFtheta}}

%bold and tilde: roman
\newcommand{\BFxtilde}{\widetilde{\BFx}}
\newcommand{\BFXtilde}{\widetilde{\BFX}}
\newcommand{\BFytilde}{\widetilde{\BFy}}
\newcommand{\BFYtilde}{\widetilde{\BFY}}
%bold and tilde: greek
\newcommand{\BFalphatilde}{\tilde{\BFalpha}}


%bar and hat: greek
\newcommand{\sigmabarhat}{\hat{\bar{\sigma}}}

%MATHSF
\newcommand{\sfm}{\mathsf{m}}
\newcommand{\sfv}{\mathsf{v}}
\newcommand{\sfw}{\mathsf{w}}
\newcommand{\sfx}{\mathsf{x}}
\newcommand{\sfz}{\mathsf{z}}

\newcommand{\sfB}{\mathsf{B}}
\newcommand{\sfH}{\mathsf{H}}
\newcommand{\sfM}{\mathsf{M}}
\newcommand{\sfV}{\mathsf{V}}
\newcommand{\sfX}{\mathsf{X}}
\newcommand{\sfZ}{\mathsf{Z}}



%MATHCAL 
\newcommand{\mcA}{\mathcal{A}}
\newcommand{\mcB}{\mathcal{B}}
\newcommand{\mcC}{\mathcal{C}}
\newcommand{\mcD}{\mathcal{D}}
\newcommand{\mcE}{\mathcal{E}}
\newcommand{\mcF}{\mathcal{F}}
\newcommand{\mcG}{\mathcal{G}}
\newcommand{\mcH}{\mathcal{H}}
\newcommand{\mcI}{\mathcal{I}}
\newcommand{\mcJ}{\mathcal{J}}
\newcommand{\mcK}{\mathcal{K}}
\newcommand{\mcL}{\mathcal{L}}
\newcommand{\mcM}{\mathcal{M}}
\newcommand{\mcN}{\mathcal{N}}
\newcommand{\mcO}{\mathcal{O}}
\newcommand{\mcP}{\mathcal{P}}
\newcommand{\mcQ}{\mathcal{Q}}
\newcommand{\mcR}{\mathcal{R}}
\newcommand{\mcS}{\mathcal{S}}
\newcommand{\mcs}{\mathcal{s}}
\newcommand{\mcT}{\mathcal{T}}
\newcommand{\mcU}{\mathcal{U}}
\newcommand{\mcV}{\mathcal{V}}
\newcommand{\mcW}{\mathcal{W}}
\newcommand{\mcX}{\mathcal{X}}
\newcommand{\mcY}{\mathcal{Y}}
\newcommand{\mcZ}{\mathcal{Z}}

%mathcal and bar
 \newcommand{\mcDbar}{\bar{\mcD}}
 \newcommand{\mcEbar}{\bar{\mcE}}
 \newcommand{\mcPbar}{\bar{\mcP}}
%mathcal and hat
\newcommand{\mcDhat}{\hat{\mcD}} 
\newcommand{\mcEhat}{\hat{\mcE}} 
\newcommand{\mcPhat}{\hat{\mcP}}
 \newcommand{\mcShat}{\hat{\mcS}}
 %mathcal and tilde
 \newcommand{\mcYtilde}{\widetilde{\mcY}}
\newcommand{\mcOtilde}{\widetilde{\mcO}}

%MATHBB 
\newcommand{\mbA}{\mathbb{A}}
\newcommand{\mbB}{\mathbb{B}}
\newcommand{\mbC}{\mathbb{C}}
\newcommand{\mbD}{\mathbb{D}}
\newcommand{\mbE}{\mathbb{E}}
\newcommand{\mbF}{\mathbb{F}}
\newcommand{\mbG}{\mathbb{G}}
\newcommand{\mbH}{\mathbb{H}}
\newcommand{\mbI}{\mathbb{I}}
\newcommand{\mbJ}{\mathbb{J}}
\newcommand{\mbK}{\mathbb{K}}
\newcommand{\mbL}{\mathbb{L}}
\newcommand{\mbM}{\mathbb{M}}
\newcommand{\mbN}{\mathbb{N}}
\newcommand{\mbO}{\mathbb{O}}
\newcommand{\mbP}{\mathbb{P}}
\newcommand{\mbQ}{\mathbb{Q}}
\newcommand{\mbR}{\mathbb{R}}
\newcommand{\mbS}{\mathbb{S}}
\newcommand{\mbT}{\mathbb{T}}
\newcommand{\mbU}{\mathbb{U}}
\newcommand{\mbV}{\mathbb{V}}
\newcommand{\mbW}{\mathbb{W}}
\newcommand{\mbX}{\mathbb{X}}
\newcommand{\mbY}{\mathbb{Y}}
\newcommand{\mbZ}{\mathbb{Z}}

%MATHFRAK
\newcommand{\mfz}{{\mathfrak{z}}}
\newcommand{\mfE}{\mathfrak{E}}
\newcommand{\mfS}{\mathfrak{S}}

%mathbb with hat
\newcommand{\mbEhat}{\hat{\mbE}}
\newcommand{\mbVhat}{\hat{\mbV}}

%%% SPACING -----------------------------------------------------------------------------

\newcommand{\spc}{\vspace{.15in}}
\newcommand{\fillpg}{\vspace*{\fill}}

%%% OPERATIONS -----------------------------------------------------------------------------

\newcommand{\defn}{\mathrel{\mathop:}=}
\newcommand{\nfed}{=\mathrel{\mathop:}}
\newcommand{\seteq}{\stackrel{\mbox{\footnotesize{set}}}{=}}


  
%%% TREATMENT OF FIGURES -----------------------------------------------------------------------------
    % Alter some LaTeX defaults for better treatment of figures:
    % See p.105 of "TeX Unbound" for suggested values.
    % See pp. 199-200 of Lamport's "LaTeX" book for details.
    %   General parameters, for ALL pages:
    \renewcommand{\topfraction}{0.9}	% max fraction of floats at top
    \renewcommand{\bottomfraction}{0.8}	% max fraction of floats at bottom
    %   Parameters for TEXT pages (not float pages):
    \setcounter{topnumber}{2}
    \setcounter{bottomnumber}{2}
    \setcounter{totalnumber}{4}     % 2 may work better
    \renewcommand{\textfraction}{0.05}	% allow minimal text w. figs
    %   Parameters for FLOAT pages (not text pages):
    \renewcommand{\floatpagefraction}{0.85}	% require fuller float pages
	% N.B.: floatpagefraction MUST be less than topfraction !!
    \renewcommand{\dblfloatpagefraction}{0.85}	% require fuller float pages

\pdfminorversion=6 

